Manifestation of the topological index formula in quantum waves and geophysical waves

Using semi-classical analysis in $\mathbb{R}^{n}$ we present a quite general model for which the topological index formula of Atiyah-Singer predicts a spectral flow with the transition of a finite number of eigenvalues between clusters (energy bands). This model corresponds to physical phenomena that are well observed for quantum energy levels of small molecules [faure_zhilinskii_2000,2001], also in geophysics for the oceanic or atmospheric equatorial waves [Matsuno_1966, Delplace_Marston_Venaille_2017] and expected to be observed in plasma physics [Qin, Fu 2022].

==> images/default <==
#FIG 3.2  Produced by xfig version 3.2.8b
Landscape
Center
Metric
A4
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 -1 -1 0.000 1 0.0000 2430 1260 445 445 2430 1260 2745 1575
2 1 2 1 0 7 50 -1 -1 3.000 0 0 -1 0 0 2
	 2430 1260 2790 990
2 1 2 1 0 7 50 -1 -1 3.000 0 0 -1 0 0 2
	 2430 1260 2970 1260
4 0 0 50 -1 0 12 0.0000 2 180 705 2790 1935 $\\theta$\001

